Privacy-Preserving Screening for Record Linkage

In an era dominated by big data and machine learning, establishing valuable data collaboration has never been more critical. However, such collaborations must operate under regulatory and legal constraints. Two-party Privacy-Preserving Record Linkage (PPRL) emerges to assess the potential collaboration value and also ensure the privacy and security of the involved data. Nevertheless, the substantial computational and communication overheads associated with PPRL hinder its practical adoption in data markets with numerous potential collaborators. Therefore, we present the Screening-then-Linkage framework, which incorporates a lightweight Screening phase prior to the resource-intensive PPRL phase, i.e., PPRS, to mitigate the scalability issue of PPRL. We propose a circuit-PSI-based system, named Appraisal to realize a secure, effective, and efficient PPRS. To reconcile the approximate matching and/or schema-aware setting required in PPRS with the limitations of the circuit-PSI supporting only symmetric functions, we propose a more communication-efficient secure permutation, i.e., Oblivious Attribute/Feature Alignment protocol tailored for PPRS. This protocol supports a broader range of comparison functions and significantly improves efficiency, i.e., reducing communication costs by a factor of 14 compared to the conventional protocol. Our rigorous analysis and comprehensive empirical evaluations demonstrate the security, effectiveness, and efficiency of Appraisal. Appraisal can accommodate up to $850\times$ more records than the SOTA PPRS system, SFour, within the same constraints. Moreover, it is $165 \times$ faster than SOTA PPRL, indicating the Screening-then-Linkage framework substantially decreases the computation time required to identify the most valuable collaborators from a large pool of candidates.

==> section/5-instantiation.tex <==
\section{PPRS Instantiation}
\label{sec:instantiation}

In this section, we will first demonstrate how \sys\ supports fuzzy matching.
Next, we will illustrate how to support both schema-aware and schema-agnostic PPRS.
Finally, we will discuss how \sys\ handles missing values.

% The definition of schema-aware and schema-agnostic is similar to the concept of blocking approach in record linkage~\cite{papadakis2015schema}.
% Formally, the schema-aware PPRS exploits a-priori schema information to leverage the most distinctive values from original or derived attributes as the key in the set intersection for finding linkage.
% In contrast, the schema-agnostic PPRS does not take any schema information into account, using all tokens from all attribute values as a key in set intersection for finding linkage.

\subsection{Supporting approximate Matching}
% Fuzzy matching is an approximate string matching approach.
% Different from exact matching where the decision of matching is binary, fuzzy matching will give a similarity score for the candidate pair and a threshold will be given to determine whether the candidate pair is matched.
% It is a common attribute in the record linkage due to there may be some errors/typos in the records, and it should be tolerant.

approximate matching is an approximate matching approach. It assigns a similarity score to the candidate pair and uses a threshold to determine whether the pair is a match. 
There are two kinds of approximate matching, 
It is commonly used in record linkage to tolerate errors or typos in records.
To support fuzzy matching, we adopt locality-sensitive hash (LSH)~\cite{indyk1998approximate}, one of the most effective approaches in record linkage~\cite{mests2018distributed,papadakis2023benchmarking}. LSH finds the nearest neighbor in high-dimensional space and outputs the same hash value if the input is similar. Among various LSH versions, we choose MinHash LSH~\cite{leskovec2020mining} because it has proven effective in the PSI scenario. MinHash LSH approximates the Jaccard coefficient between derived sets from candidate record pairs.
In particular, a string will be split into a set, $E$, of all overlapping substrings with a given length, denoted as $q-grams$, where $q$ is the length of the substring.
Then for each q-gram string $e$, LSH applies $B\cdot R$ different MinHash functions, \ie,
$min_{e\in E} \mathsf{H}(e)$.
The results are separated into $B$ bands of $R$ digests, then the concatenation of the $R$ digests will be hashed as the signature of the band.
Finally, a candidate attribute pair is matched iff one of the band signatures is matched.

To implement this approach in \sys, the \emph{attribute Engineering} component works as follows: 
(i) $P_0$ and $P_1$ synchronize the parameters $B$ and $R$, as well as the metadata of attributes.
(ii) They extract $q$-grams from the attribute values $X_j$. 
(iii) Each party generates a new $\bar{X}$ by expanding one record to $B$ band signatures, increasing the number of attribute from $m$ to $Bm$. 
(iv) Both parties run the \emph{Circuit-PSI} and \emph{OFA} components to obtain the aligned set intersection result.

The \emph{Score Function} component works as follows: Since the attribute of each record has been expanded to $B$ signatures, the determination of whether the attribute $j$ is matched is calculated via $\lor_{k=j\cdot B}^{(j+1)B-1}\langle \bar{Q}_{k}\rangle$

% the score of one record is calculated as $\langle s_i \rangle = \sum_{j=i\cdot B}^{(i+1)B-1}{\mathsf{B2A}(\bar{Q}_{i})}$, and the decision can be calculated via $\langle d_i \rangle = \mathsf{MSB}(s_i>T_B)$.

% To support fuzzy matching, we adopt locality-sensitive hash (LSH)~\cite{indyk1998approximate}, one of the most effective approaches in record linkage~\cite{mests2018distributed,papadakis2023benchmarking}.
% It tries to find the nearest neighbor in the high-dimension space, and outputs the same hash value if the input is similar to each other.
% There are different versions of LSH, such as MinHash LSH~\cite{leskovec2020mining}, Hyperplane LSH~\cite{charikar2002similarity}, Cross-Polytope LSH~\cite{lv2007multi}, \etc
% Among them, we choose MinHash LSH because it has been proven effective in PSI scenario~\cite{adir2022privacy}.
% In general, MinHash LSH approximates the Jaccard coefficient between the derived sets from the candidate record pair.

% In particular, a string will be split into a set, $E$, of all overlapping substrings with a given length, denoted as $q-grams$, where $q$ is the length of the substring.
% Then for each q-gram string, LSH applies $B\cdot R$ different MinHash functions, \ie,
% $min_{e\in E} \mathsf{H}(e)$.
% The results are separated into $B$ bands of $R$ digests, then the concatenation of the $R$ digests will be hashed as the signature of the band.
% The LSH is the list of the $B$ band signatures.
% Finally, for a candidate record pair, if there are more than a threshold $T_B$ of band signatures from this pair are the same, then we consider it as a matched pair.

% To implement such an approach in \sys, \emph{attribute Engineering} component works as follows:
% $P_0$ and $P_1$ first synchronize the parameters $B, R$ as well as the metadata of attributes.
% Then they will extract $q-grams$ from the attribute value $X_j$;
% Then each party generates a new $\bar{X}_j$ by expanding one record to $B$ band signatures, \ie, the number of the attribute value expands from $n$ to $Bn$.
% Next, both parties run \emph{Circuit-PSI} and \emph{OFA} components to get the aligned set intersection result.
% The \emph{Score Function} components work as follows:
% Since each record has been expanded to $B$ values of signatures, the determination of whether the record is linked should be calculated based the continues $B$ intersection result.
% Specifically, the score of one record $s_i = \sum_{k=i\cdot B}^{(i+1)B-1}{\mathsf{B2A}(\bar{Q}_{i})}$ and the decision can be calcualted via $\mathsf{MSB}(s_i>T_B)$.

\subsection{Supporting Distance-based Matching}
~\cite{andoni2015practical}

\subsection{Schema-aware PPRS}
In schema-aware PPRS, a-priori schema information is used to leverage the most distinctive values from original or derived attributes as the key in the set intersection for finding linkage. 
The metadata of the data, such as the name of the attribute and the format, should be public to support this mode. The \emph{attribute Engineering} works as follows:
Firstly, $P_0$ and $P_1$ synchronize the attributes used in PPRS. However, directly using some attributes will be ineffective. For example, the gender attribute, as the values ``male'' and ``female'' appear in both $X^1$ and $X^0$. Therefore, to reduce the false positive rate, new attributes should be derived or existing attributes should be concatenated. The approach to deriving new attributes can be determined empirically, and parties should synchronize this.
After $P_0$ and $P_1$ derive new attributes, if the derived attributes have some errors or typos, they should be preprocessed via MinHash LSH-based fuzzy matching. After all this preprocessing, they can run one instance of Circuit-PSI for each derived attribute $\bar{X}^0_{_,j}$ and $\bar{X}^1_{_,j}$.

% the schema-aware PPRS exploits a-priori schema information to leverage the most distinctive values from original or derived attributes as the key in the set intersection for finding linkage. 
% In schema-aware PPRS, the metadata of the data, such as the name of the attribute and the format, should be public.
% To support such mode, the \emph{attribute Engineering} works as follows:

% Firstly, $P_0$ and $P_1$ synchronize the attribute used in the PPRS.
% However, directly using of some attributes will be useless. 
% For example, the gender because the value of male and female for the attribute appears in both $X^1$ and $X^0$.
% Thus, we should derive some new attributes or concat the attributes to reduce the false positive rate.
% The approach to deriving new attributes could be determined empirically, and parties should synchronize this.

% After $P_0$ and $P_1$ deriving new attributes, if the derived attribute has some errors/typos, it should also preprocess via MinHash LSH-based for fuzzy matching.
% After all this preprocessing, they can run one instance of Circuit-PSI for each derived attribute $\bar{X}^0_{\_,j}$ and $\bar{X}^1_{\_,j}$.

\subsection{Schema-agnostic PPRS}
The schema-agnostic PPRS does not consider any schema information, using all tokens from all attribute values as a key in set intersection to find linkages. This can be easily implemented by concatenating all values from different attributes into one long string.
Specifically, in the \emph{attribute Engineering} component, %two parties 
$P_0$ and $P_1$ do the following: Firstly, they synchronize the attributes they use, and then concatenate the values into one attribute.
It is worth noting that our approach essentially transforms the matching problem into a set intersection with exact matching. Therefore, directly inputting the long attribute into the Circuit-PSI could lead to low accuracy. We encourage the use of other attribute engineering techniques simultaneously in this setting, \eg, MinHash LSH to improve accuracy.

% The schema-agnostic PPRS does not take any schema information into account, using all tokens from all attribute values as a key in set intersection for finding linkage.
% It could be easily implemented by concating all values from different attributes into one long string.
% Specifically, in the \emph{attribute Engineering} component, two parties $P_0$ and $P_1$ does following:
% Firstly, $P_0$ and $P_1$ should synchronize the attribute they used, and then concat the values to be one attribute.
% However, our approach essentially transforms the matching problem to be the set intersection with exact matching.
% Thus, directly inputting the long attribute to the Circuit-PSI could lead to low accuracy.
% We encourage to using other attribute engineering techniques simultaneously in this setting, such as the MinHash LSH.

\subsection{Handling Missing Value}

In many cases, the data is incomplete, meaning that some attribute values are missing. 
% Handling missing values is relatively straightforward in PPRL due to the rich comparison function used in their system. However, 
In Circuit-PSI, the output is limited to two kinds of values: match or unmatch. Consequently, if the data is input into Circuit-PSI without intentionally processing the missing values, all missing attributes will be ultimately determined as a match, leading to a high false positive rate.

We observe that the receiver ($P_0$ in this paper) of the Circuit-PSI will know which values are missing because it inserts the data via Cuckoo hash and knows the $\pi^c$. Thus, it can adjust the missing value score for each record in the \emph{Score function} component.
Let's take the linear/logistic model as an example. We denote the weight for missing values as $w^m_j$ for attribute $j$. After both parties calculate $\langle s\rangle^A$, if the attribute value $\bar{X}_{i,j}$ is missing, $P_i$ can locally adjust the score $\langle s_i\rangle^A = \langle s_i\rangle^A + w^m_j$.


% In many cases, the data is incomplete, \ie, with some missing attribute value.
% It can be easily handled in PPRL due to the rich comparison function used in their system.
% However, the Circuit-PSI can only output two kinds of value: match or unmatch. 
% Thus, if the data is input into Circuit-PSI without intentional processing the missing value, all missing attributes will be ultimately determined as match, leading to a high false positive rate.

% We observe that the receiver ($P_0$ in this paper) of the Circuit-PSI will know which value is missing, because it inserts the data via Cuckoo hash and knows the $\pi^c$.
% Thus, it can adjust the missing value score for each record in \emph{Score function} component.

% Let's take the linear/logistic model as an example, we denote the weight for missing is $w^m_j$ for attribute $j$.
% After both parties calculate the $\langle s\rangle^A$, if attribute value $\bar{X}_{i,j}$ is missing, $P_i$ locally adjust the score $\langle s_i\rangle^A = \langle s_i\rangle^A + w^m_j$

==> section/8-discussion.tex <==
\section{Discussion}

\subsection{How to link record after screening}
If both parties' dataset have all the exact matching attribute and have no repeat values of any attribute. The screening can be converted to link record. In particular, 

\subsection{How to find the weights and threshold in linear/logistic model~\ref{sec:score_records}}
Assume that the probability of $j$-th attribute of two linked record mapping into the same bin is $p_{1,j}$, and the probability of $j$-th attribute of two non-linked record mapping into the same bin is $p_{2,j}$. The weights $w_i$ and threshold $t$ should satisfy $E_1> t> E_2$, where
\begin{align*}
E_1 = & \sum_{\delta_1,\delta_2,\cdots,\delta_m\in\{0,1\}}(\sum_{j=1}^mw_j\delta_j)\prod_{j=1}^mp_{1,j}^{\delta_j}(1-p_{1,j})^{1-\delta_j}, \\
E_2 = & \sum_{\delta_1,\delta_2,\cdots,\delta_m\in\{0,1\}}(\sum_{j=1}^mw_j\delta_j)\prod_{j=1}^mp_{2,j}^{\delta_j}(1-p_{2,j})^{1-\delta_j}. \\
\end{align*}
For $j$-th attribute being comparable, $p_{1,j}=1$ and $p_{2,j}=0$. Otherwise, using $(r,cr,p_1,p_2)$-sensitive LSH hash to assign the values of $j$-th attribute into distinct bins. At this time, $p_{1,j}$ is regarded as the similarity probability $p_1$, and $p_{2,j}$ is regarded as the non-similarity probability $p_2$. If the attribute has missing value, then $p_{1,j}$ should be reduced by missing rate. If the attribute has repeat value, then $p_{2,j}$ should be added by repetition rate. Note that the value $\frac{E_1}{E_2}$ is larger, the weights $w_i$ is better. Therefore, $t$ can be exactly $\frac{E_1+E_2}{2}$.

